xSemAD: Explainable Semantic Anomaly Detection in Event Logs Using Sequence-to-Sequence Models

The identification of undesirable behavior in event logs is an important aspect of process mining that is often addressed by anomaly detection methods. Traditional anomaly detection methods tend to focus on statistically rare behavior and neglect the subtle difference between rarity and undesirability. The introduction of semantic anomaly detection has opened a promising avenue by identifying semantically deviant behavior. This work addresses a gap in semantic anomaly detection, which typically indicates the occurrence of an anomaly without explaining the nature of the anomaly. We propose xSemAD, an approach that uses a sequence-to-sequence model to go beyond pure identification and provides extended explanations. In essence, our approach learns constraints from a given process model repository and then checks whether these constraints hold in the considered event log. This approach not only helps understand the specifics of the undesired behavior, but also facilitates targeted corrective actions. Our experiments demonstrate that our approach outperforms existing state-of-the-art semantic anomaly detection methods.

==> sections/notes.tex <==




\begin{table}[!tb]
\centering
\resizebox{1\columnwidth}{!}{
\centering
    \begin{tabular}{P{3cm}P{3cm}P{3cm}P{2cm}P{2cm}P{2cm}} 
    \toprule
    Scope & Approach & Setting & Precision & Recall & $F_{1}$\\
     \midrule
     \multirow{3}{6em}{Test set}&
     SVM\cite{caspary2023does}& &  0.54 & 0.74 & 0.58 \\
     & BERT\cite{caspary2023does}& & 0.54 & 0.74 & 0.58\\
     & label2rule &$T$=0.73 & 0.63 & \textbf{0.78} & \textbf{0.67}\\ & label2rule &with individual $T$ & \textbf{0.64} & 0.76 & \textbf{0.67}\\  
     \bottomrule
     \multirow{3}{6em}{Only models with unseen labels}&
     SVM\cite{caspary2023does}& &  \textbf{0.54} & 0.69 & 0.56 \\
     & BERT\cite{caspary2023does}& & \textbf{0.54} & 0.69 & 0.56\\
     & label2rule &$T$=0.73 & 0.52 & \textbf{0.73} & \textbf{0.57}\\
     & label2rule &with individual $T$ & \textbf{0.54} & 0.71 & \textbf{0.57}\\ 
     \bottomrule
     \end{tabular}
}
\vspace{2mm}
\caption{eventually-follows relations: performance comparison of SVM, BERT, and our approach under different scenarios}
\label{tbl:results-comparison}
\end{table}




\begin{table}[!tb]
\centering
\resizebox{1\columnwidth}{!}{
\centering
    \begin{tabular}{P{3cm}P{3cm}P{3cm}P{2cm}P{2cm}P{2cm}} 
    \toprule
    Scope & Approach & Setting & Precision & Recall & $F_{1}$\\
     \midrule
     \multirow{3}{6em}{Test set}&
     SVM\cite{caspary2023does}& &  0.54 & 0.74 & 0.58 \\
     & BERT\cite{caspary2023does}& & 0.54 & 0.74 & 0.58\\
     & label2rule &$T$=0.73 & 0.63 & \textbf{0.78} & \textbf{0.67}\\ & label2rule &with individual $T$ & \textbf{0.64} & 0.76 & \textbf{0.67}\\  
     \bottomrule
     \multirow{3}{6em}{Only models with unseen labels}&
     SVM\cite{caspary2023does}& &  \textbf{0.54} & 0.69 & 0.56 \\
     & BERT\cite{caspary2023does}& & \textbf{0.54} & 0.69 & 0.56\\
     & label2rule &$T$=0.73 & 0.52 & \textbf{0.73} & \textbf{0.57}\\
     & label2rule &with individual $T$ & \textbf{0.54} & 0.71 & \textbf{0.57}\\ 
     \bottomrule
     \end{tabular}
}
\vspace{2mm}
\caption{eventually-follows relations: performance comparison of SVM, BERT, and our approach under different scenarios}
\label{tbl:results-comparison}
\end{table}





\begin{figure}[!htbp]
     \centering
         \centering
         \includegraphics[width=70mm]{figures/evaluation_sap_sam_2022_test_label2constraint_for_comparison_overall_performance.pdf}
         \caption{overall - test set blabla}
         \label{fig:sd}
\end{figure}

\begin{figure}[!htbp]
     \centering
         \centering
         \includegraphics[width=70mm]{figures/evaluation_sap_sam_2022_validation_label2constraint_for_comparison_set.pdf}
         \caption{eventually-follows - validation set blabla}
         \label{fig:sadfhgf}
\end{figure}




\section{Fine-tuning}
%The automatic generation of constraints based on the given event labels $\mathcal{E}$ requires an approach that takes into account the semantic relationships between the events in a process. 
%To accomplish this task we fine tuned a sequence-to-sequence model in the (1) component, to be more specific we used Flan-T5~\cite{flant5}. Flan-T5 is a pre-trained language model that was trained on a variety of supervised and unsupervised tasks. We fine-tune Flan-T5 for constraint generation by training it on data from a large process model repository $\mathcal{M}$, specifically on input-target pairs. The trained model can then be used when applying the approach on any event log.

For generating the training dataset we first need to specify the input-target samples. The input value is given by the unique event labels in a process. 

%Let $\mathcal{M}$ be a process model repository containing $n$ distinct processes, given as $P_i$ for $1 \leq i \leq n$. and let $E_i$ represent the set of event labels for process $P_i$, and $e_{ij}$ denote the $j$-th occurrence of the event label in $E_i$. Thus, a process $P_i$ can be expressed as:
%$P_i = \{e_{i1}, e_{i2}, \ldots, e_{in_i}\}$,
%where $n_i$ is the total number of unique and repeated event labels in process $P_i$.


The input value of a training sample is given by the set of unique event labels $U_i$ in a process:
$U_i = \{e_{ij} \mid e_{ij} \in E_i \text{ and } e_{ij} \neq e_{ik} \text{ for } j \neq k\}$.
%Thus, $U_i$ represents the unique event labels present in the process $P_i$, which serve as the input value for our input-target training pairs.

The target value of a training sample is defined by a constraint with which $U_i$ is trained.
To get our target values we defined and extracted constraints for each process model $P_i$. We make use of the declarative process language \textit{declare}~\cite{DiCiccio2022} and define the following constraints:
\begin{enumerate}
    \item \textbf{Initiation constraint:} $\text{{init}}(e_{j})$ -- The process starts with event $e_{j}$.
    \item \textbf{Termination constraint:} $\text{{end}}(e_{j})$ -- The process ends with event $e_{j}$.
    \item \textbf{Succession constraint:} $\text{{succession}}(e_{j}, e_{k}) \equiv e_{j} \rightarrow_{s} e_{k}$ -- Event $e_{j}$ ($e_{k}$) occurs if and only if it is followed (preceded) by event $e_{k}$ ($e_{j}$) in the process instance.
    \item \textbf{Alternate Succession constraint:} $\text{{alt\_succession}}(e_{j}, e_{k}) \equiv e_{j} \leftrightarrow e_{k}$ -- Events $e_{j}$ and $e_{k}$ occur in the process instance if and only if the latter follows the former, and they alternate each other in the trace.
    \item \textbf{Choice constraint:} $\text{{choice}}(e_{j}, e_{k}) \equiv e_{j} \lor e_{k}$ -- Either event $e_{j}$ or event $e_{k}$ must be in the process.
    \item \textbf{Co-existence constraint:} $\text{{coexistence}}(e_{j}, e_{k}) \equiv e_{j} \land e_{k}$ -- Both events $e_{j}$ and $e_{k}$ must be in the process.
    \item \textbf{Exclusive Choice constraint:} $\text{{exclusive\_choice}}(e_{j}, e_{k}) \equiv e_{j} \oplus e_{k}$ -- Either event $e_{j}$ or event $e_{k}$ (but not both) must be in the process.
    \item \textbf{Response constraint:} $\text{{response}}(e_{j}, e_{k}) \equiv e_{j} \rightarrow_{r} e_{k}$ -- If event $e_{j}$ occurs in the process instance, then event $e_{k}$ occurs after $e_{j}$.
    \item \textbf{Alternate Response constraint:} $\text{{alt\_response}}(e_{j}, e_{k}) \equiv e_{j} \rightarrow (e_{k} \land e_{j})$ -- Each time event $e_{j}$ occurs in the process instance, event $e_{k}$ occurs afterwards, before $e_{j}$ recurs.
    \item \textbf{Precedence constraint:} $\text{{precedence}}(e_{j}, e_{k}) \equiv e_{j} \rightarrow_{p} e_{k}$ -- Event $e_{k}$ occurs in the process instance only if preceded by event $e_{j}$.
    \item \textbf{Alternate Precedence constraint:} $\text{{alt\_precedence}}(e_{j}, e_{k}) \equiv e_{k} \rightarrow  e_{j} \land (\lnot e_{k} \mathit{U} e_{j})$ -- Each time event $e_{k}$ occurs in the process instance, it is preceded by event $e_{j}$, and no other $e_{k}$ can recur in between.
\end{enumerate}
However, we emphasize that our approach also works independently of these specific constraint types and that our approach can be extended with additional constraint types.

\begin{definition}[Training sample, training dataset]
For each process $P_i$ in the model repository $\mathcal{M}$, the set of constraints is given by $\mathcal{R}_i = \{R_{i1}, R_{i2}, \ldots, R_{im_i}\}$, where $m_i$ is the total number of constraints associated with $P_i$. Each constraint $R_{ik}$ is categorized into a specific constraint type (e.g., initiation, choice or response), denoted as $T_{ik}$. We define a training sample as a input-target pair $(T_{ik}:\text{{shuffle}}(U_i), R_{ik})$, where $1 \leq k \leq m_i$, representing the set of unique event labels in $P_i$ and one constraint selected from the set of constraints associated with $P_i$. 
We randomize the order of $(U_i)$ in each training sample by $\text{{shuffle}}(U_i)$. 
This ensures the model remains unbiased by the order of event labels, compelling it to focus on learning the intrinsic relationships among these labels.
We then define the entire training dataset as the union of all training samples:
$\mathcal{M}_{train} = \bigcup_{i=1}^{n} \{(T_{ik}:\text{{shuffle}}(U_i), R_{ik}) \mid U_i \text{ is the set of unique event labels in } P_i, R_{ik} \in \mathcal{R}_i, T_{ik} \text{ is the constraint type of } R_{ik}\}.$
\end{definition}
%For each process $P_i$ in the model repository $\mathcal{M}$, the set of constraints is given by $\mathcal{R}_i = \{R_{i1}, R_{i2}, \ldots, R_{im_i}\}$, where $m_i$ is the total number of constraints associated with $P_i$. Each constraint $R_{ik}$ is categorized into a specific constraint type (e.g., initiation, choice or response), denoted as $T_{ik}$. We define a training sample as a input-target pair $(T_{ik}:\text{{shuffle}}(U_i), R_{ik})$, where $1 \leq k \leq m_i$, representing the set of unique event labels in $P_i$ and one constraint selected from the set of constraints associated with $P_i$. 
%We randomize the order of $(U_i)$ in each training sample by $\text{{shuffle}}(U_i)$. 
%This ensures the model remains unbiased by the order of event labels, compelling it to focus on learning the intrinsic relationships among these labels.
%We then define the entire training dataset as the union of all training samples:
%$\mathcal{M}_{train} = \bigcup_{i=1}^{n} \{(T_{ik}:\text{{shuffle}}(U_i), R_{ik}) \mid U_i \text{ is the set of unique event labels in } P_i, R_{ik} \in \mathcal{R}_i, T_{ik} \text{ is the constraint type of } R_{ik}\}.$
We use this training dataset $\mathcal{M}_{train}$ to fine-tune Flan-T5. 

To illustrate that, two possible training sample for the simplified application handling process in Fig BLA would be:

- (Init: check, receive application, reject application, approve application, pay compensation; Init(receive application)

- (Exclusive choice: approve application, receive application, check, reject application, pay compensation; Exclusive choice(approve application, reject application)



\mypar{Generate constraints}
The fine-tuned Flan-T5 model has the ability to autonomously create constraints based on event labels.
This functionality extends the applicability of the model to various event logs. 
The constraint creation process involves entering a sequence into our fine-tuned model. This sequence includes a constraint type $T_{k}$, that specifies the type of constraint to be created, and the associated event labels $\mathcal{E}$ extracted with the \textit{ExtractLabels} function in the event-label extractor.
Our model uses a strategy where $n$ output sequences corresponding to $n$ potential constraints are generated for a given input. This is achieved by applying \textit{beam search}~\cite{graves2012sequence}, which serves as a decoding mechanism for our fine-tuned model.
One limitation of the beam search algorithm is its tendency to generate output sequences with repeated words or short patterns. Consequently, the output may contain event names that are very similar to the intended names.
To ensure that we only consider constraints with valid event labels, we narrow down the selection to only those event names that were originally present in the input sequence. 
To further refine the output, we introduce a threshold parameter called $T$. This threshold plays a crucial role in determining the set of constraints. Only constraints with a probability above the defined threshold are considered for output. This step increases the precision of the generated constraints by filtering out constraints with lower probabilities.

To illustrate, consider the event log in the example above with event labels \textit{check, accept application, reject application, receive application}. If the goal is to determine possible start events (the corresponding declare constraint would be \textit{init}) based on the event labels, the corresponding input sequence for our model would be as follows: \textit{(init: check, accept application, reject application, receive application)}. 
In this example, the input sequence specifies the constraint type as "Init" and provides a list of event labels extracted using the \texttt{ExtractLabels} function in the event-label extractor. Our model uses the beam search algorithm to generate potential constraints based on this input sequence. Consider the three generated output sequences:
\begin{enumerate}
    \item "Init: receive application"
    \item "Init: check"
    \item "Init: receive request"
\end{enumerate}
We filter out the third output sequence because it contains "receive request", which was not in the original input sequence. The beam search algorithm uses conditional probabilities to track the most likely output sequences at each generation step. Suppose the probabilities for the remaining two constraints are:

\begin{enumerate}
    \item "Init: receive application" - Probability: 0.95
    \item "Init: check" - Probability: 0.40
\end{enumerate}
Consider a threshold $T= 0.7$. Since the second constraint has a probability below the threshold, it is filtered out, and the final generated constraint is "Init: receive application", i.e., based on the given labels the process should begin with the event \textit{receive application}.
This example illustrates the constraint generation process. 
The various constraints can now be created by changing the constraint type in the input sequence. 


\mypar{Anomaly Detector}
After the constraint generation phase, where semantic constraints capturing relationships between event labels are derived, the next step in our approach is anomaly detection. In this phase, the generated constraints are applied to the event log to identify instances of semantic violations, i.e., situations where the observed process deviates from the specified constraints.

\mypar{Anomaly Detection Process} The anomaly detection process involves the application of the generated constraints to the event log. The result of this process is a set of detected semantic violations that indicate where the observed behavior of the trace deviates from the expected constraints. The first step in the anomaly detection process is the application of constraints.
The set of constraints $\mathcal{R}$ generated in the constraint-generation phase is applied to the event log $\mathcal{L}$. This is done by using an anomaly detector, which checks each trace in the event log against the set of constraints to identify instances of constraint violations.
Second, for each trace in the event log, the anomaly detector identifies if any of the constraints have been violated. A violation occurs when the observed sequence of events in a trace contradicts the constraints established for the process. The result of this step is a set of instances where semantic violations have been detected.
Thirdly, the anomaly detector provides information on which specific constraints have been violated as soon as violations are detected. This explanatory capability is crucial for understanding the nature of the anomaly and facilitates the process of addressing and correcting the issues in the process.
The final output of the anomaly detection phase is a set $V$ of detected semantic violations. Each instance in this set corresponds to a trace in the event log where a violation of the derived semantic constraints has been identified. The anomaly detector not only flags these violations but also associates them with the specific constraints that have been breached.

\mypar{Illustration} To illustrate, consider the event log and constraints generated in the previous example. Suppose the event log contains the following trace:

$\tau_{4}=<$\textit{check, accept application, pay compensation}$>$

In this case, the anomaly detector, utilizing the generated constraints, would identify that the trace $\tau_{4}$ violates the constraints. Specifically, it violates the constraint derived from the example: the application should start with the \textit{receive application} event. The anomaly detector would output a detected semantic violation for trace $\tau_{4}$ and indicate that it violates the constraint "Init: receive application."

This explanatory capability of the anomaly detection phase provides stakeholders with insights into where and why the process deviates from the expected behavior, enabling a more informed and targeted approach to addressing anomalies in the system.





\begin{enumerate}
    \item \textit{Initiation constraint:} $\text{{init}}(a_{j})$ -- The process starts with activity $a_{j}$.
    \item \textit{Termination constraint:} $\text{{end}}(a_{j})$ -- The process ends with activity $a_{j}$.
    \item \textit{Succession constraint:} $\text{{succession}}(a_{j}, a_{k}) \equiv a_{j} \rightarrow_{s} a_{k}$ -- Activity $a_{j}$ ($a_{k}$) occurs if and only if it is followed (preceded) by activity $a_{k}$ ($a_{j}$) in the process.
    \item \textit{Alternate Succession constraint:} $\text{{alt\_succession}}(a_{j}, a_{k}) \equiv a_{j} \leftrightarrow a_{k}$ -- Activities $a_{j}$ and $a_{k}$ occur in the process if and only if the latter follows the former, and they alternate each other in the trace.
    \item \textit{Choice constraint:} $\text{{choice}}(a_{j}, a_{k}) \equiv a_{j} \lor a_{k}$ -- Either activity $a_{j}$ or activity $a_{k}$ must be in the process.
    \item \textit{Co-existence constraint:} $\text{{coexistence}}(a_{j}, a_{k}) \equiv a_{j} \land a_{k}$ -- Both activities $a_{j}$ and $a_{k}$ must be in the process.
    \item \textit{Exclusive Choice constraint:} $\text{{exclusive\_choice}}(a_{j}, a_{k}) \equiv a_{j} \oplus a_{k}$ -- Either activity $a_{j}$ or activity $a_{k}$ (but not both) must be in the process.
    \item \textit{Response constraint:} $\text{{response}}(a_{j}, a_{k}) \equiv a_{j} \rightarrow_{r} a_{k}$ -- If activity $a_{j}$ occurs in the process, then activity $a_{k}$ occurs after $a_{j}$.
    \item \textit{Alternate Response constraint:} $\text{{alt\_response}}(a_{j}, a_{k}) \equiv a_{j} \rightarrow (a_{k} \land a_{j})$ -- Each time activity $a_{j}$ occurs in the process instance, activity $a_{k}$ occurs afterwards, before $a_{j}$ recurs.
    \item \textit{Precedence constraint:} $\text{{precedence}}(a_{j}, a_{k}) \equiv a_{j} \rightarrow_{p} a_{k}$ -- Activity $a_{k}$ occurs in the process instance only if preceded by activity $a_{j}$.
    \item \textit{Alternate Precedence constraint:} $\text{{alt\_precedence}}(a_{j}, a_{k}) \equiv a_{k} \rightarrow  a_{j} \land (\lnot a_{k} \mathit{U} a_{j})$ -- Each time activity $a_{k}$ occurs in the process instance, it is preceded by activity $a_{j}$, and no other $a_{k}$ can recur in between.
\end{enumerate}





\begin{table}[!tb]
\begin{center}
\scriptsize
\begin{tabular}{ c l  c  c  c c  c  c c  c  c c  c  c c  c  c}
\toprule
%\hline
&\textbf{Scenario} & \multicolumn{3}{c}{\textbf{SVM}\cite{caspary2023does}} & \multicolumn{3}{c}{\textbf{BERT}\cite{caspary2023does}}& \multicolumn{3}{ c }{\textbf{MINERful}\cite{ciccio2015discovery}}& \multicolumn{3}{ c }{\textbf{DecM}\cite{maggi2012efficient}}& \multicolumn{3}{ c }{\textbf{xSemAD}} \\ 
%\cline{2-5}
& & Prec. & Rec. & $F_1$& Prec. & Rec. & $F_1$& Prec. & Rec. & $F_1$& Prec. & Rec. & $F_1$ & Prec. & Rec. & $F_1$ \\
\midrule

(ii)&EvF-UD &0.32&0.61&0.40 & 0.32&0.61&0.40 & 0.32&0.60&0.40 & 0.32&0.60&0.40& \textbf{0.53}&\textbf{0.74}&\textbf{0.58}\\ 
\midrule
(iii)&Init& - & - & - & - & - & - &0.20 & \textbf{0.79} & 0.31 & \textbf{0.70} &0.77 &\textbf{0.71}& 0.37 & 0.60 & 0.43\\ 

&End& - & - & - & - & - & - &0.24 & 0.72 & 0.34 &0.58 &\textbf{0.64}& \textbf{0.59}& \textbf{0.50} & 0.57 & 0.49\\ 

&Resp& - & - & - & - & - & - &0.05 & \textbf{0.50} & 0.09 &0.08&\textbf{0.50}&0.12& \textbf{0.22} & 0.36 & \textbf{0.25}\\ 
&AltResp& - & - & - & - & - & - &0.05 & \textbf{0.50} & 0.09 &0.01& 0.03& 0.01& \textbf{0.20} & 0.39 & \textbf{0.24}\\ 
&Succ & - & - & - & - & - & - & 0.12 & \textbf{0.60} & 0.18 & - & - & - &\textbf{0.25} & 0.49 & \textbf{0.29}\\ 
&AltSucc & - & - & - & - & - & - &0.12 & \textbf{0.60} & 0.18 & - & - & - &\textbf{0.24} & 0.53 & \textbf{0.29}\\ 
&Prec & - & - & - & - & - & - &   0.10&\textbf{0.62}&0.16 &0.14 &0.61 &0.21& \textbf{0.26} & 0.59 & \textbf{0.32}\\ 
&AltPrec & - & - & - & - & - & - & 0.10&\textbf{0.62}&0.16 &0.02 &0.04& 0.02& \textbf{0.24} & 0.61 & \textbf{0.31}\\ 
&Ch & - & - & - & - & - & - &- & - & - &0.14 &\textbf{0.59}& 0.22& \textbf{0.29} & 0.54 & \textbf{0.34}\\ 
&ExCh & - & - & - & - & - & - &- & - & - & - & - & - &\textbf{0.25} & \textbf{0.59} & \textbf{0.31}\\ 
&CoEx  & - & - & - & - & - & - & 0.28 & 0.61 & 0.35&- & - & - & \textbf{0.43} & \textbf{0.68} & \textbf{0.47}\\ 
\bottomrule
\end{tabular}
\end{center}
\caption{Performance comparison of SVM, BERT, Minerful, DecM, and xSemAD across different scenarios.}
\label{tbl:results-comparison}
\end{table}
